A Review of Privacy and Consent Management in Healthcare: A Focus on Emerging Data Sources

The emergence of New Data Sources (NDS) in healthcare is revolutionising traditional electronic health records in terms of data availability, storage, and access. Increasingly, clinicians are using NDS to build a virtual holistic image of a patient's health condition. This research is focused on a review and analysis of the current legislation and privacy rules available for healthcare professionals. NDS in this project refers to and includes patient-generated health data, consumer device data, wearable health and fitness data, and data from social media. This project reviewed legal and regulatory requirements for New Zealand, Australia, the European Union, and the United States to establish the ground reality of existing mechanisms in place concerning the use of NDS. The outcome of our research is to recommend changes and enhancements required to better prepare for the 'tsunami' of NDS and applications in the currently evolving data-driven healthcare area and precision or personalised health initiatives such as Precision Driven Health (PDH) in New Zealand.

==> sections/standards.tex <==
\section{National and Global Standards}
In national standards, we study aspects and rules that might have an effect on privacy and patient consent in New Zealand.First, we do a review of the Health Information Security Framework (HISO 10029:2015)  of New Zealand, which specifies the information security policies and guidelines that should be implemented by healthcare providers to address the maintaining Confidentiality, Integrity and Availability of patient’s healthcare data.

We also do a review of global standards, i.e., International Organization for Standardization (ISO) to understand the requirements and standards that are set out concerning EHR and consent. ISO has a wide coverage on different guidelines and standards for health informatics. In this section, we focus specifically on consent and data privacy. One term that is used to define consent in ISO standards is Informational Consent, where it refers to consent for the patient information, as opposed to Consent for Treatment, where the captured consent is specifically for the treatment.


\subsection{National standards}
HISO 10029:2015 gives a provides a general consent assumption where it “assumes personal health information will be shared – it does not say what information is to be shared or under what circumstances” \cite{HISO-NZ}. However, there is an emphasis on making sure that patient data is de-identified and making sure that there is a protection in place for identified patient data during transit and at rest, this is achieved by implementing cryptographic functions to encrypt the data. This will lead to more concerns about key management and storage of data, especially on cloud computing services which are gaining prominence \cite{HISO-NZ}.
 
There is a provision in HISO 10029:2015 for cloud computing which states that the minimum security coverage as transmission, storage, processing of information, encryption and decryption of data, recovery of data, and third party access to information. The main concern when using a cloud computing service is when data is being stored or processed in a cloud infrastructure, where the cryptographic key to which the data is encrypted on the cloud server and that the data and key will not be misused or disseminated \cite{HISO-NZ}.

HISO defines access control as a way to stop unauthorised access to confidential healthcare information and access rights must be defined as ‘least rights’ until given access by an approver, which in this case is an administrator after reviewing patient consent documents. A periodic review of each access right granted must be done to ensure that there is no prolonged access that will compromise privacy \cite{HISO-NZ}. HISO is based on the traditional RBAC (Role-based access control), which does not include patients ability to view or approve access control rights for PHR. The Personal Health Working Group (PWHG), defines PHR as  “an electronic application through which individuals can access, manage and share their health information, and that of others for whom they are authorized, in a private, secure, and confidential environment” \cite{Markle-PHR}. This differs from EHR, where the access is generally limited to healthcare professionals and is not shared with patients. 

The initial assumption of data being shared by HISO makes it difficult to implement NDS based on the currently suggested HISO framework because NDS is very private in nature, should be only used with patient agreement in the right context.

\subsection{ISO Standards}
ISO/TS 17975:2015 \cite{ISO-17975-2015}defines a set of frameworks of consent for collection, use or disclosure of personal health information. The standards define consent and give a guideline of consent framework and mechanisms. It also makes a distinction between Informational Consent and consent to treatment. 

ISO/TS 14441:2013 \cite{ISO-14441-2013} defines privacy requirements for EHR systems. It defines the requirements for recording Informational Consent, minimum data to be recorded, and emergency access allowance.

ISO/TS 14265:2011 \cite{ISO-14265-2011}defines the range of purposes for which personal health data might be used in treatments and where Informational Consent might be required.

ISO/TS 25237:2008 \cite{ISO-25237-2008}is a specification on pseudo-anonymisation methodologies of personal health information are covered in the standards as well as statistical tests to determine the effectiveness of pseudo-ano
nymisation.

ISO 27799:2016 \cite{ISO-27799-2016} provides guidelines to information security for healthcare. It includes Informational Consent requirements for policy implementation, electronic messaging, access privilege assignment, and data protection and privacy.

The reviewed ISO guidelines and technical standards would help to define more clearly how informational consent framework should be managed and captured and would serve as a baseline to patients giving their NDS as a source of data to improve healthcare. 

\subsection{Health Level 7 (HL7)}

HL7 is a set of defined standards for transfer of clinical administrative information between different applications used by healthcare providers. It defines standard terminologies and formats for message and data exchange, rules, and health data definitions.

Under HL7, Fast Healthcare Interoperability Resources (FHIR) \cite{HL7} is a standard developed to describe data formats and APIs for health record exchange on the web. FHIR builds on existing versions of HL7 and allows for backwards compatibility. FHIR works well with OAuth defining standard resource Uniform Resource Locator (URL) or web address for each medical workflow use case. This will allow OAuth to be able to redirect users with tokens to only specific URLs.

FHIR serves as the baseline to standardise messaging across different patient portals, allowing patients to delegate information to their healthcare provider.




==> sections/systems.tex <==
\section{Existing Healthcare Systems}

We have also done an extensive literature review on the current systems access control methods and how they are used in healthcare systems in different countries. To this end, we have studied healthcare systems used worldwide with focus on New Zealand, Australia  Singapore, UK, Italy, and USA. We identify strengths and weaknesses of existing healthcare systems and investigate how we can leverage them to propose a New Zealand healthcare system based on current legislation.

 \subsection{New Zealand healthcare}
New Zealand has 20 District Health Boards (DHBs), each one having autonomy on what software they use to store clinical data but it has the highest uptake of EHR systems. 

New Zealand has achieved 99.9\% EHR penetration since 2000 \cite{EMR-Adoption}, but with regards to consent capturing, traditional forms and verbal consent are still the way it is done. With regards to current New Zealand consent to PHR, it is an implied consent and there is currently no opt out option for EHR and there is also no way to control the roles and access to patient’s data, logs are unavailable to patients as well but patients can request for their PHR from their respective DHB by filling out a form \cite{ADHB-EHR}.

New Zealand has a fragmented database problem, making it difficult to reconcile data across DHBs. There is also a problem on GP referral to hospitals because the software used is different and stored locally, a hard copy of the records would have to be transferred. In the event of cross DHB referrals, e.g., Waikato DHB to Auckland DHB, electronic referral and exchange of information are not possible because of the different software vendors used. DHBs would still have to re-key a hard copy or electronic copy into their own systems \cite{Deloitte-report}

Findings: 
Most existing systems lack the ability to either offer patients a fine-grained access control mechanism, or a holistic log of their medical data. A trade-off between security, ease of use, and access must be made to ensure that it is easily accessible and used between all groups and ages. Existing systems are not able to contextually add information from other data sources, this would be invaluable information from a medical standpoint.

 \subsection{Australian Healthcare System (My Health Record)}
 Australia’s My Health Record is based on identity-based access control \cite{My-Health-Record}, where the government has set up their own Public Key Infrastructure (PKI) called Nash PKI. This is PKI that guarantees that only recognised health providers would have a private key and able to digitally sign messages ensuring their identity. 
\newline
The server generates a Personal Access Code (PAC), which is sent to the patient that can be shared with healthcare providers ensuring that only people who have the PAC can access the patient’s data. The PAC expires after 30 days, and there are logs that users are able to check to see what information was accessed and when \cite{My-Health-Record}.

The default setting allows anyone with PAC to view all the patient’s data but patients are able to set access control on what data is available and add their own data by “flagging specific documents in your record as ‘limited access’, and controlling who can view these documents” \cite{My-Health-Record}.

\subsection{Singapore National Electronic Health Record (NEHR)}

While Singapore has a concise and holistic traditional healthcare database implemented, because it is a small state country it was easier to compile data between hospitals and ensure that they have agreed on one single framework. However, they lack privacy for the following reasons:
\begin{itemize}
\item An implied-consent, patients will have to opt out of it if needed.
\item The RBAC model requires custom roles for each level. This system assumes all clinicians have the same role, any GP/healthcare provider can access patient data as long as they have basic patient information [8]. This will not work in New Zealand, as it violates health information privacy act .
\item According to Section 6 Principle 3 of the New Zealand Privacy Act 1993 \cite{1993-privacy}, “the agency shall take such steps (if any) as are, in the circumstances, reasonable to ensure that the individual concerned is aware of (information collected and used)”.  Ideally, the patient’s consent must be captured before collecting/accessing information, a general implied opt-in RBAC such as the one implemented in Singapore violates the privacy of the patient.
\end{itemize}

\subsection{UK National Health Service (NHS)}
The UK NHS \cite{NHS-SCR} follows the RBAC model and is based on smart cards, whereby the smart cards are assigned to healthcare personnel depending on their role. This is basically a 2-factor authentication where only specific terminals fitted with specialised card reader and software can access the database \cite{NHS-HealthRec}.

Although it is mentioned in \cite{SCR-LPC} that “consent must be explicitly given to healthcare personnel”, but consent capturing process is vague and verbal consent is also acceptable. It lacks a verification step, where health care personnel can always say that they have gained the user’s consent and there is no way to verify this. The consent capturing process still uses a manual form \cite{SCR-LPC}.

Summary Care Records (SCRs) do not contain an overall medical record of the patient; as the name suggests, it is only a summary of important patient records.Summary Care Record is a summary of patient information, which contains allergies, adverse reactions and current medications given to the patient [18] It lacks other detailed reports and history about the patient.PHR is not available to patients at the moment, but patients can request a copy from their GP or local pharmacist.

\subsection{Italian Healthcare System}
Patients in Italy are given a health care card (“Tessera Sanitaria” in Italian), which is essentially a smart card for health insurance, where patients will be assigned unique identifiers with the card that will allow them to login into the system and view their PHR [17].

Informed consent is a major requirement in their health care legislation [12], however how consent should be captured is not defined [31]. Consent is divided into two categories in the Italian EHR, a general consent stating that the patient agrees to setup the EHR and then a specific consent granting healthcare providers access to the patient’s EHR [31].The guidelines [31] also make allowance for consent revocation; however, it does not mention how this is done. The EHR guidelines [31] distinguishes data into two types of data, minimum dataset, which contains medical and first aid reports, discharge information, must be made available at a regional level and other data sets, which might not be included in referrals depending on the completeness of the region’s dataset. 

\subsection {Massachusetts MedRec}
This system is based on Blockchain technology \cite{zyskind_nathan_pentland_2015}, which offers auditability and provides a holistic view of who accessed patient data \cite{azaria_medrec:_2016}. Apparently, such a complex technology might require a lot computing resources. Access control in MedRec uses a smart contract, this works in the same way as a normal contract, where there are a set of rules that will be enforced. In this case, smart contracts would be used to define relationships and also access, but it involves a link across contracts and setting rules that will only allow authorised persons to view and update data. 



